A Simple Approach for Visual Rearrangement: 3D Mapping and Semantic Search

Physically rearranging objects is an important capability for embodied agents. Visual room rearrangement evaluates an agent's ability to rearrange objects in a room to a desired goal based solely on visual input. We propose a simple yet effective method for this problem: (1) search for and map which objects need to be rearranged, and (2) rearrange each object until the task is complete. Our approach consists of an off-the-shelf semantic segmentation model, voxel-based semantic map, and semantic search policy to efficiently find objects that need to be rearranged. On the AI2-THOR Rearrangement Challenge, our method improves on current state-of-the-art end-to-end reinforcement learning-based methods that learn visual rearrangement policies from 0.53% correct rearrangement to 16.56%, using only 2.7% as many samples from the environment.

==> sections/checklist.tex <==
\section*{Checklist}
% Examples:
%\answerNA{}
%\answerNo{The code and the data are proprietary.}
%\answerYes{See Section~\ref{gen_inst}.}
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Sections~\ref{sec:method} and \ref{sec:rearrangement}}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:failure}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code will be released upon acceptance. See Algorithm~\ref{alg:mass} for pseudo-code. Section~\ref{sec:exp} contains notes on existing data set RoomR for AI2-THOR Rearrangement Challenge. Details about hyperparameters and tuning are given in Appendix~\ref{app:hyperparameters}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details about hyperparameter tuning and training details are given in Appendix~\ref{app:hyperparameters}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{While the official challenge leaderboard (performance reported in the Table~\ref{tab:leaderboard} and Table~\ref{tab:componentwise_ablation}) does not expose error bars, we have conducted an additional performance comparison in Appendix~\ref{app:errorbars} that includes error bars. }
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details about necessary compute are available in Appendix~\ref{app:compute}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{sec:exp}}
  \item Did you mention the license of the assets?
    \answerNo{The original dataset RoomR was released under Apache License 2.0. See \href{https://github.com/allenai/ai2thor-rearrangement}{https://github.com/allenai/ai2thor-rearrangement}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{No new data.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{RoomR was released under Apache 2.0 license.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> sections/intro.tex <==
% TODO 

% CSR Introduction structure by paragraph for reference:
% 1. scene representation is important
% 2. scene graphs are a good option but have limitations
% 3. discrete set of relationships has limitations
% 4. another limitation of scene graphs is that they are static
% 5. to address this limitation of scene graphs we present CSR
% 6. our method constructs the scene representation interactively using object relational embeddings
% 7. we show experimentally that our method is good

%\gunnar{
%Preliminary introduction structure suggestion. Message by paragraph:
%\begin{enumerate}
%    \item Understanding the scene is critical for robotics tasks, including rearrangement
%    \item RL methods start from scratch and are faced with a overly challenging learning problem; performance on rearrangement is quite low
%    \item If the semantic map is known, the task is easy
%    \item We focus on constructing a good semantic map
%    \item our method does XYZ
%    \item We show experimentally that our method is good
%\end{enumerate}
%}

%\gunnar{made a quick draft of the intro do fill in the blanks, feel free to discard it completely}
%Brandon.2022.05.16: I edited this paragraph to focus on motivating why we should care about rearrangement as a skill, and why its hard.

% Understanding the scene is critical for robotics tasks, including rearrangement
%Physically rearranging objects is an important skill for %embodied agents to aid humans in the real world. Early works %like \cite{BenShahar1996PracticalPP} showed how rearrangement %requires understanding the 3D environment, but this remains an %immense practical challenge for embodied agents, confirmed by %the difficulty of recent benchmarks \citep{embodiedqa, %ALFRED20, batra2020rearrangement, weihs2021visual}. Knowledge %of the 3D environment is at the heart of various tasks for %embodied agents, such as point navigation~\citep{anderson18}, %image navigation~\citep{Batra2020ObjectNavRO,Yang2018VisualSN}, vision language %navigation~\citep{Anderson2018VisionandLanguageNI,ALFRED20}, 
%embodied question %answering~\citep{gordon18,embodiedqa}, and 
%more. Effective %scene representations that enable planning 
%and decision-making %in complex 3D environments have broad 
%relevance across these %tasks for embodied agents, and is 
%especially important for %visual 
%rearrangement~\citep{batra2020rearrangement,weihs2021visual}. 
%Rearrangement problems are defined by a set of objects, %and a 
%set of corresponding object goal configurations. %Rearrangement is especially challenging because an effective %agent must generalize to a combinatorially large number of %object locations and states. Successful agents must identify %the locations and states of each object to properly understand %the rearrangement goal. This is a challenging embodied %perception task that depends on a scene representation that %effectively describes the information necessary to rearrange %objects.

\gunnar{agree with Ben's comments about streamlining this section. The last part about rearrangement being challenging could maybe more streamlined to be: (1) this is the task, (2) this is why it's difficult. The current version goes a bit back and forth.}

\gaurav{agree with Ben and Gunnar, hence see modified intro and related work below.}

Rearrangement problems are defined by a set of objects, and a set of corresponding object goal configurations. They are especially challenging because an effective agent must generalize to a combinatorially large number of object locations and states. Successful agents must identify the locations and states of each object to properly understand the rearrangement goal. This is a challenging embodied perception task that depends on a scene representation that effectively describes the information necessary to rearrange objects.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{assets/rearrangement_teaser3.pdf}
    \caption{\textbf{Our method incrementally builds a voxel-based map from observations.} This visualization shows the 3D voxel map built by our method after mapping and searching in the observation phase. The colors are obtained by assigning each class a different color (background class gray) and using a weighted average from the class probabilities. For example, we can see the laptop on the bed (pink), book on the bed (blue), and clock on the drawers (yellow). In the rearrangement phase an analogous map is built, and the discrepancies between the two maps are used to solve the rearrangement problem. We visualize an example rearrangement on the right with the initial position of the pink object (laptop on the bed), followed by the agent holding the object (laptop), and finally the destination position of the object (laptop on the desk). 
    \gunnar{initial version of the teaser idea, using a visualization of a learned map.}}
    \label{fig:teaser}
\end{figure}

% RL methods start from scratch and are faced with a overly challenging learning problem; performance on rearrangement is quite low
%Brandon.2022.05.16: I edited this paragraph to focus on where the paradigm of coupling RL with broadly scaled experience can go wrong.
In many embodied learning tasks, the standard approach is reinforcement learning (RL) with broadly scaled experience~\citep{weihs2021visual,chaplot2020neural,DBLP:journals/corr/abs-2104-04112}. In a simulated environment with unlimited retries, this experience is cheap to obtain, and agents can be trained with random exploration until a good solution is discovered by the agent. This pipeline works incredibly well for tasks like point navigation~\citep{Wijmans2020DDPPOLN}, but in some cases this strategy is not enough. As the difficulty of embodied learning tasks increases, the agent must generalize to an increasing number of environment configurations, and broadly scaled experience becomes insufficient. For example, when \cite{weihs2021visual} scale their agent to 75 million environment steps, end-to-end RL still only rearranges 0.53\% of objects correctly in Table~\ref{tab:leaderboard}. Without a scene representation that effectively describes objects, end-to-end RL may not be enough to solve visual rearrangement.

% If the semantic map is known, the task is easy
In the rearrangement setting, a hypothetical perfect understanding of the environment makes the problem almost trivial: an object A is location X, and should go to location Y. Visual rearrangement can be readily solved if perfect information about the locations and states of objects is available to the agent in an accessible format. Our initial experiments suggest that accurate 3D semantic maps of the environment are one such accessible format for visual rearrangement. With accurate 3D semantic maps, our method rearranges 15.11\% of objects correctly, and requires significantly less experience from the environment to do so. %While end-to-end RL requires up to 75 million environment steps in \cite{weihs2021visual}, our method only requires 2 million samples and trains offline. 
Our results suggest an important question: can we prioritize understanding the environment over end-to-end RL? 
%\gunnar{Brandon, can you verify these numbers, and maybe mention a part of the experiments where we show this? (ablations?)}
%Brandon.2022.05.16: done, I modified the number, and also made some edits to the presentation. The original message was already pretty good.

% We focus on constructing a good semantic map
%We want to make semantic mapping work better in dynamic environments. Where dynamic means that elements of the environment can move (like furniture), and certain objects can have a state (like a door). We solve a set of visual navigation tasks that require understanding the state of the environment in order to successfully complete the task goal.
%We focus on determining if we can improve the semantic segmentation and improve detection of map disagreement between the rearrangement phases.

% Our method does XYZ
%This work proposes a simple alternative for rearrangement: (1) Search for objects that need to be rearranged, and (2) rearrange each object until the task is complete. 
%While simple, we show that we can utilize an off-the-shelf semantic segmentation model to improve a voxel-based semantic map. This map can then be used to directly inform a semantic search policy to efficiently find objects that need to be rearranged.

% We show experimentally that our method is good
%We demonstrate that our method can obtain significant gains on the both visually and geometrically complex task of the 2022 AI2-THOR Rearrangement Challenge~\cite{weihs2021visual}. Our method outperforms current state-of-the-art by 30.2 times despite requiring 37.5 times fewer environment transitions to reach this performance. Our approach is simple, efficient, and effective at visual rearrangement despite being trained offline.

%Brandon.2022.05.16: the goal of this paragraph is to lead in to our contributions (the next paragraph) by talking about what our method does.
We demonstrate how semantic maps help agents effectively understand dynamic 3D environments and perform visual rearrangement. These dynamic environments have elements that can move (like furniture), and objects with changing states (like the door of a cabinet). We present a method that builds accurate semantic maps in these dynamic environments, and reasons about what has changed. Deviating from prior work that leverages end-to-end RL, we propose a simple approach for visual rearrangement: (1) search for and map which objects need to be rearranged, and (2) procedurally rearrange objects until a desired goal configuration is reached. We evaluate our approach on the AI2-THOR Rearrangement Challenge \cite{weihs2021visual} and establish a new state-of-the-art.

%Brandon.2022.05.16: the goal of this paragraph is to list our specific contributions.
Our contributions include an architecture for visual rearrangement that builds voxel-based semantic maps of the environment, and rapidly finds objects using a semantic-search policy. Our approach is flexible, and shows a robustness to a variety of object sizes and rearrangement goal difficulties. Our experimental evaluation shows an improvement of 13.21 absolute percentage points over current work in visual rearrangement: an additional 396 / 3004 objects rearranged. \gunnar{I'm not sure the 396/3004 number is easy enough to understand to be impressive here.} We conduct ablations to diagnose where the bottlenecks are for visual rearrangement, and find that accurate scene understanding is most crucial. With a perfect semantic map, our method solves 38.33\% of tasks, improving by 36.13 absolute percentage points over prior work \textit{in the same regime}. Our results suggest voxel-based semantic maps are an effective scene representation for visual rearrangement, and semantic-search is an effective tool for building accurate semantic maps with a limited navigation budget.

==> sections/method.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{assets/neurips2022_main_diagram.pdf}
    \caption{Our method incrementally builds a voxel-based \emph{Semantic Map} from observations. The semantic map is compared with the map from the observation phase, and used to either follow the \emph{Semantic Search Policy}, or apply a list of \emph{Rearrangement Policies}. \gunnar{Do we need a separate ``Teaser Figure''? This might be more suited as "Figure 2: The Model Figure"}}
    \label{fig:main_diagram}
\end{figure}

In this section, we present a simple baseline for visual room rearrangement. Our method consists of a voxel-based semantic map representation of the scene, and a high-level semantic search policy that locates which objects to rearrange as fast as possible. Figure~\ref{fig:main_diagram} illustrates how these components interact. We begin this section by discussing the decision-making setting our method operates in, and how our method functions in this setting. Consider the room rearrangement problem defined by \cite{batra2020rearrangement}, which is a special case of a Markov Decision Process (MDP). Rearrangement problems are defined in terms of a set of objects to be rearranged, and a set of goal configurations for those objects with which the task is considered solved. The goal of a rearrangement agent is to successfully rearranging all objects in the environment to their goal configurations. Our approach reaches this goal by imposing additional structure on the observation space. Our method observes egocentric RGB and depth images, and the agent's pose. These observations are used to actively constructive a voxel-based semantic map \gunnar{should we cite something for the voxel-based semantic map?} that informs the agent where objects are located in the scene. Our map provides an effective memory of the scene that helps the agent infer the rearrangement goal of the environment by visually observing the room in its goal configuration. In the next section, we will detail how the semantic map is constructed, and how it integrates with our search policy.

\begin{algorithm}[h]
\caption{3D Mapping \& Semantic Search For Rearrangement}\label{alg:mapping_algorithm}
\begin{algorithmic}
\Require environment $e$, voxel-based maps $m_c, m_n \in \mathcal{R}^{H \times W \times D \times C}$, navigation steps $T$, pre-trained Mask R-CNN $g$, semantic search policy $\pi_{\theta}$
\Function{BuildSemanticMap}{$m_c$, $m_n$, $e$, $g$, $T$}
\For{$t \gets 1$ to $T$}                    
    \State image$_t$, depth$_t$, pose$_t$ $\gets$ $e$.get\_observations()
    \State ind$_t$ $\gets$ get\_voxel\_indices$($ depth$_t$, pose$_t$ $)$
    \State $m_c [$ ind$_t$ $]$ $\gets$ $m_c [$ ind$_t$ $]$ + $g($ image$_t$ $)$ \Comment aggregate semantic predictions in map
    \State $m_n [$ ind$_t$ $]$ $\gets$ $m_n [$ ind$_t$ $]$ + 1 \Comment count number of hits per voxel
    \State $a_t$ $\gets$ SemanticSearch( $m_c / m_n$, pose$_t$)
\EndFor
\EndFunction
\Function{SemanticSearch}{$m_c$, pose$_t$}
  \If{goal$_t$ is reached or goal$_t$ does not exist}
    \State goal$_t$ $\gets$ $\pi_{\theta}$($m_c$) \Comment emit semantic search goal
  \EndIf
  \State \Return navigation\_action(goal$_t$, pose$_t$) \Comment execute planner
\EndFunction
\end{algorithmic}
\end{algorithm}

\gunnar{should we maybe call the observation map just $m$, the counts $n$, and normal map $m^*$? (trying to reduce indices). Could also use $\mathcal{M}, \mathcal{N}, \mathcal{M}^*$}

Our \textit{Semantic Mapping} algorithm, shown in Algorithm~\ref{alg:mapping_algorithm}, is based on \cite{DBLP:conf/nips/ChaplotG0S20}. \gunnar{Should we clarify how it is different here?} We incrementally build a map of the scene at every timestep, using RGB and depth images, and pose. The semantic map $m_c$ is a 4-tensor, corresponding to a vector of semantic class probabilities for each voxel in a 3D grid. The size of the voxel grid, represented by grid height $H$, width $W$, and depth $D$, is chosen to accommodate the largest scenes we test our method on. In practice, we use 5cm voxels arranged in a grid of height 384, width 384, and depth 96, which accommodates scenes as large as 40 meters in height and width. Given the latest RGB and depth images, and pose, we model the agent as a pinhole camera and update the semantic map $m_c$ by projecting rays into the scene from the camera through the center of each pixel in the imaging plane. Using the depth image, we terminate rays at a distance corresponding to a pixel's depth. This is shown in Equation~\ref{eqn:voxel_indices}, where the matrix $R\in\mathcal{R}^{3 \times N}$ represents a batch of rays for $N$ pixels in the imaging plane, $d\in\mathcal{R}^{N}$ represents the depth of each pixel, $T\in\mathcal{R}^{3 \times 3}$ represents the rotation matrix from the camera coordinate system to the world coordinate system, and $b\in\mathcal{R}^{3}$ represents the location of the camera in the world coordinate system. Using evenly spaced voxels of length $c$, we then compute in which voxel each ray terminates. 
\begin{equation}\label{eqn:voxel_indices}
    \text{ind}_t = \left \lfloor \left( T R \text{diag}( \mathbf{d} )  + 1^{T} \mathbf{b} \right) / c \right \rfloor + \lfloor H/2 \rfloor
\end{equation}
\gunnar{this equation could probably be done for a single pixel at a time, and simplified by assuming the ray $r$ is given e.g. $\text{ind}_t^i = \left \lfloor (b_t + d_t^i r_t^i) / c \right \rfloor$ and assuming we handle the indices properly in our tensor implementation (maybe no need for H/2)}
These indices delineate which voxels we are observing by each pixel at the current timestep. We use the indices in Algorithm~\ref{alg:mapping_algorithm} to update the semantic map $m_c$ by adding the vector of class probabilities returned by a perception model for every pixel. We additionally record the number of observations for each voxel in a second map $m_n$, which we use to normalize $m_c$. This normalization has the affect of averaging the observations for each voxel, which helps filter the predictions of an imperfect perception model to improve the map quality. During exploration, the semantic map is updated at every timestep. To build a complete map, especially when scenes are large, sufficient exploration of the environment is needed. We accomplish this by selecting navigation goals using a \textit{Semantic Search} policy $\pi_{\theta}$ that conditions on the partial semantic map $m_c$. The semantic search policy leverages the partial map to choose locations of the environment to observe that are likely to contain objects that need to be rearranged. Once a navigation goal is selected, we use path planning to reach it.
\begin{equation}\label{eqn:voxel_indices}
    \max_{\theta} \mathbb{E}_{\tau} \left[ \sum_{i = 1}^{H} \sum_{j = 1}^{W} \tilde{p}_{\tau}(i, j) \log \pi_{\theta}( m_c (\tau) )[i, j] \right] : \; \tilde{p}_{\tau}(i, j) \propto \frac{1}{K} \sum_{k = 1}^{K} \mathcal{N}([i, j]^{T}; \mu_{\tau,k}, \sigma^2 I)
\end{equation}
\gunnar{might be cleaner as two lines of equations. $\tau$ wasn't used before this and makes the equation a bit messy. Maybe it could be a superscript? Maybe the policy could be written as $ \pi_{\theta}(i, j | m_c )$ etc}
\brandon{I agree. I needed a way to indicate the ground truth distribution changes depending on the contents of the room, which is a random variable.}
The semantic search policy $\pi_{\theta}$ is trained with supervised learning using a ground truth search distribution $\tilde{p}_{\tau}(i, j)$. This distribution is a two-dimensional mixture of Gaussians, with a Gaussian mode centered at each of the $K$ objects in scene $\tau$ that need to be rearranged. The position vector $[i, j]^{T}$ represents a top-down location in the scene. The mean of each Gaussian mode $\mu_{\tau,k}$ represents the top-down location of the kth object in the scene to rearrange, and the standard deviation $\sigma$ is a hyperparameter that controls the stochasticity of the semantic search policy. Once the semantic search policy is trained, navigation goals sampled from it encode a semantic prior for object locations in the scene that accelerates finding the objects to rearrange. 
\gunnar{we might be missing some details on the semantic search policy $\pi_\theta$, is there a citation we should be using? Are there conv layers etc? It might not be completely clear how this policy is used at inference time, for example, how does it use the map tensor?}
We leverage Dijkstra's algorithm \citep{dijkstra1959note} for planning a path from the agent's current location to navigation goals at runtime.

\begin{algorithm}[h]
\caption{Multi-Episode Semantic Search For Rearrangement}\label{alg:rearrange_algorithm}
\begin{algorithmic}
\Require first environment $e_w$, second environment $e_u$, voxel-based maps $m_c^{\; w}, m_n^{\; w}, m_c^{\; u}, m_n^{\; u} \in \mathcal{R}^{H \times W \times D \times C}$, navigation steps $T$, pre-trained Mask R-CNN $g$, semantic search policy $\pi_{\theta}$
\State BuildSemanticMap($m_c^{\; w}$, $m_n^{\; w}$, $e_w$, $g$, $T$) \Comment this semantic map encodes the goal state
\State BuildSemanticMap($m_c^{\; u}$, $m_n^{\; u}$, $e_u$, $g$, $T$) \Comment rearrange this environment to the goal state
\While{a disagreement $d$ between $m_c^{\; w}$ and $m_c^{\; u}$ is detected}
\State navigate to the location of object $d$ in $e_u$
\State rearrange\_disagreement($d$) \Comment move and open the object if necessary
\EndWhile
\end{algorithmic}
\end{algorithm}

\brandon{
I need to explain this second algorithm box. Should we focus this section more on our novelty, and avoid going into such depth about the 3D mapping algorithm? This would save space. I'm not yet sure what's in scope for the reader.
}
\gunnar{I think this is a good level of depth so far. It's a lot easier to start with a complete explanation and then trim it where needed than knowing exactly what the right level is (also easier for us to help scope it when we have the complete picture). The section might be missing some emphasis on the novelty however, for example how the mask-rcnn is used, how the observations are combined, and making it a bit more obvious where the novel things are.}

\gunnar{It might be a bit confusing that there are two different "semantic searches", one for "exploration" and the other for rearrangement. We might need to think about how to clarify that. Maybe clarify if the same $\pi_\theta$ is used etc}


%\subsection{Scene-level Disagreement Detection}

%\brandon{
%Detail how objects are matched between phases, perhaps leave this in the appendix. 
%}

